DISCRET: Synthesizing Faithful Explanations For Treatment Effect Estimation

Designing faithful yet accurate AI models is challenging, particularly in the field of individual treatment effect estimation (ITE). ITE prediction models deployed in critical settings such as healthcare should ideally be (i) accurate, and (ii) provide faithful explanations. However, current solutions are inadequate: state-of-the-art black-box models do not supply explanations, post-hoc explainers for black-box models lack faithfulness guarantees, and self-interpretable models greatly compromise accuracy. To address these issues, we propose DISCRET, a self-interpretable ITE framework that synthesizes faithful, rule-based explanations for each sample. A key insight behind DISCRET is that explanations can serve dually as database queries to identify similar subgroups of samples. We provide a novel RL algorithm to efficiently synthesize these explanations from a large search space. We evaluate DISCRET on diverse tasks involving tabular, image, and text data. DISCRET outperforms the best self-interpretable models and has accuracy comparable to the best black-box models while providing faithful explanations. DISCRET is available at https://github.com/wuyinjun-1993/DISCRET-ICML2024.

==> Sections/Motivation.tex <==
\section{Motivating examples}

% comparing against post-hoc explanations
In this section, we present some motivating examples in Figure \ref{fig: motivating_example} to highlight the necessity of enforcing consistency property on explanations and shed light on the impact of consistent explanations on prediction performance. To accomplish this. in Figure \ref{fig: motivating_example}, we focus on three samples from the test split of \ihdp\ dataset and their explanations produced by two baselines, Causal Forest \citep{athey2019estimating} and Anchor \citep{ribeiro2018anchors}, and \ours\ respectively. Note that Causal Forest is a self-interpretable method for treatment effect estimation while Anchor is one broadly used rule-based post-hoc explanation method. Here we employ Anchor to interpret the predictions by one state-of-the-art treatment effect estimation model, TransTEE \citep{zhang2022exploring}. In addition to the explanations produced by these methods, the corresponding predicted individual treatment effect (ITE) values are also reported (we report the predicted values by TransTEE for Anchor).


Ideally, since explanations reflect how a machine learning model performs predictions, one would expect that the samples with identical explanations would be associated with nearly the same predicted results. This property is termed consistency, which has been regarded as one critical criterion for measuring explanation faithfulness \citep{dasgupta2022framework}.
However, as Figure \ref{fig: motivating_example} suggests, although the explanations produced by Anchor are equivalent for the sample $x_2$ and $x_3$, the TransTEE model yields distinct and inaccurate predictions for these two samples (their ground truths are 4.25 and 4.78 respectively while the predicted values are both less than 3.75). This thus raises concerns about the reliability of such explanations. In contrast, \ours\ explicitly enforces the consistency constraints over the generated explanations and the predicted ITE values as introduced in Section \ref{sec: intro}. As a consequence, $x_2$ and $x_3$ not only share the same explanations but also obtain more consistent and accurate estimated ITEs, thus enhancing the faithfulness of explanations. 
% which are also close to the  This  
% Plus, the predicted ITE values by \ours\ are also the same for those two samples. Such  However, due to the lack of such consistency guarantees, the explanations generated by Anchor for the sample $x_2$ and $x_3$ fail to match the same predictions performed by the TransTEE model, which also incurs a larger gap against the ground truth in comparison to that by \ours. 

It is noteworthy that the state-of-the-art self-interpretable models, such as the decision tree-like models for general classification tasks and the causal forest model for the treatment effect estimation task, also perform predictions based on rule-based explanations, thus inherently maintaining consistency property. However, as indicated in Figure \ref{fig:example}, despite consistent explanations generated by the Causal forest model on sample $x_1$ and $x_3$, the corresponding predicted ITE value (4.5) significantly deviates from the ground truth of $x_1$. This suggests that the state-of-the-art self-interpretable models may fail to accurately capture the consistency between explanations and ground truth, thus deteriorating the prediction performance. 


% in the state-of-the-art post-hoc explanations and its correlations with poor ITE prediction performance. We also show some examples to point out that despite the self-consistency that the state-of-the-art self-interpretable models maintain, they mostly capture unreasonable consistency from the data, thus deteriorating the prediction performance. 





% comparing against other self-interpretable explanations they are self-consistent, but the ground-truths are not. capturing consistency in a wrong manner. 


